LIRA: A Learning-based Query-aware Partition Framework for Large-scale ANN Search

Approximate nearest neighbor search is fundamental in information retrieval. Previous partition-based methods enhance search efficiency by probing partial partitions, yet they face two common issues. In the query phase, a common strategy is to probe partitions based on the distance ranks of a query to partition centroids, which inevitably probes irrelevant partitions as it ignores data distribution. In the partition construction phase, all partition-based methods face the boundary problem that separates a query's nearest neighbors to multiple partitions, resulting in a long-tailed kNN distribution and degrading the optimal nprobe (i.e., the number of probing partitions). To address this gap, we propose LIRA, a LearnIng-based queRy-aware pArtition framework. Specifically, we propose a probing model to directly probe the partitions containing the kNN of a query, which can reduce probing waste and allow for query-aware probing with nprobe individually. Moreover, we incorporate the probing model into a learning-based redundancy strategy to mitigate the adverse impact of the long-tailed kNN distribution on search efficiency. Extensive experiments on real-world vector datasets demonstrate the superiority of LIRA in the trade-off among accuracy, latency, and query fan-out. The codes are available at https://github.com/SimoneZeng/LIRA-ANN-search.

==> sections/related_work.tex <==
\section{Related Work}
Existing studies for ANN search can be roughly divided into four groups, including (1) hash-based~\cite{tian2023db, huang2015query, deng2024learning}, (2) tree-based~\cite{echihabi2022hercules, guttman1984r, muja2014scalable, azizi2023elpis}, (3) quantization-based~\cite{lu2024knowledge, aguerrebere2023similarity, gao2024rabitq}, and (4) graph-based~\cite{lu2021hvs, wang2021comprehensive, malkov2018efficient, fu2021high}.
% [TO Do] 这一段可以考虑放到 related work
Typically, 
the computational cost of retrieval $k$ approximate nearest neighbors, $O(nd)$, incurs from the number of visited vectors denoted as $n$ and the dimension of vectors represented as $d$.
The existing ANN search methods leverage high-dimensional indexes to reduce latency from these two aspects.

% To reduce $d$, the quantization-based indexes~\cite{paparrizos2022fast} and hash-based indexes~\cite{tian2023db, wang2021mp} both map the original high-dimensional vectors into low-dimensional codes.

% while 

\subsection{Partition-based ANN methods}
The tree-based indexes~\cite{echihabi2022hercules} partition the vector space into nested nodes and then narrow down the search area with hierarchical tree-based indexes during the search phase.
DB-LSH et.al~\cite{tian2023db} efficiently generate candidates by dynamically constructing query-based search areas.
IVF (inverted file) index~\cite{johnson2019billion} first clusters the vectors into partitions and then narrows down the search area with the nearest partitions.
Chen et.al~\cite{chen2021spann} uses a clustering algorithm and the inverted index to build balanced posting lists, and probes the clusters within a certain distance from the query vector.
Zhang et.al~\cite{zhang2023learning} focuses on multi-probe ANN search and formalizing the query-independent optimization as a knapsack problem.
Neural LSH~\cite{dong2019learning} generates partitions by balanced graph partitioning.
Zhao et.al~\cite{zhao2023towards} combine the strength of LSH-based and graph-based methods and utilize LSH to provide a high-quality entry point for searching in graphs.


\subsection{Learning-based ANN methods}
Artificial Intelligence(AI) has been widely applied to databases~\cite{wang2017survey, li2021ai, liang2024dace, chen2023leon}, information retrieval systems~\cite{li2022deep} and decision-making scenarios~\cite{zeng2023target, hu2024imitation, fang2024efficient, xia2024parameterized, deng2022efficient}.
We provide some learning-based ANN on top of partitions and graphs.
For partition-based methods,
BLISS~\cite{gupta2022bliss} and Li et.al~\cite{li2023learning} combine the partition step and the learning step with learning-to-index methodology, and then search with a fixed $nprobe$.
Zheng et.al~\cite{zheng2023learned} builds hierarchical balanced clusters and further leverages neural networks to generate adaptive $nprobe$ for each query.
For graph-based methods,
the graph-based indexes~\cite{wang2021comprehensive, malkov2018efficient} first connect the similar vectors with basic proximity graphs in the construction phase and then route in the graph through the most similar neighbors with the greedy search strategy.
Based on the graph-based HNSW, Li et.al~\cite{li2020improving} demonstrate that easy queries often need less search depth than hard ones.
Li et.al~\cite{li2020improving} introduces an early termination strategy and uses models to predict the minimum number of visited vectors required for retrieving the ground truth $k$NN for a given query, which can halt the search before meeting the traditional termination condition in the graph.






